OKAMI: Teaching Humanoid Robots Manipulation Skills through Single Video Imitation

We study the problem of teaching humanoid robots manipulation skills by imitating from single video demonstrations. We introduce OKAMI, a method that generates a manipulation plan from a single RGB-D video and derives a policy for execution. At the heart of our approach is object-aware retargeting, which enables the humanoid robot to mimic the human motions in an RGB-D video while adjusting to different object locations during deployment. OKAMI uses open-world vision models to identify task-relevant objects and retarget the body motions and hand poses separately. Our experiments show that OKAMI achieves strong generalizations across varying visual and spatial conditions, outperforming the state-of-the-art baseline on open-world imitation from observation. Furthermore, OKAMI rollout trajectories are leveraged to train closed-loop visuomotor policies, which achieve an average success rate of 79.2% without the need for labor-intensive teleoperation. More videos can be found on our website https://ut-austin-rpl.github.io/OKAMI/.

==> related_work_submission_.tex <==
OKAMI: Teaching Humanoid Robots Manipulation
Skills through Single Video Imitation
Jinhan Li1† Yifeng Zhu1∗ Yuqi Xie1,2∗ Zhenyu Jiang1,2∗ Mingyo Seo1
Georgios Pavlakos1 Yuke Zhu1,2
UT Austin1 NVIDIA Research2
Abstract: We study the problem of teaching humanoid robots manipulation skills
by imitating from single video demonstrations. We introduce OKAMI, an algo-
rithm that generates a manipulation plan from a single RGB-D video and derives
a policy for execution. At the heart of our approach is object-aware retargeting,
which enables the humanoid robot to mimic the human motions in an RGB-D
video while adjusting to different object locations during deployment. OKAMI
uses an open-world vision pipeline to identify task-relevant objects and retarget
the body motions and hand poses separately. Our experiments show that OKAMI
achieves strong generalizations across varying visual and spatial conditions, out-
performing the state-of-the-art baseline on open-world imitation from observa-
tion. Furthermore, OKAMI rollout trajectories are leveraged to train closed-loop
visuomotor policies, which achieve an average success rate of 79.2%
need for labor-intensive teleoperation. More videos can be found on our website
https://ut-austin-rpl.github.io/OKAMI/.
Keywords: Humanoid Manipulation, Imitation From Videos, Motion RetargetingSingle Video
Imitation
Human
Demo
Human
Demo
Human
Demo
Human
Demo
Figure 1: OKAMI enables a human user to teach the humanoid robot how to perform a new task by providing
a single video demonstration.
1 Introduction
Deploying generalist robots to assist with everyday tasks requires them to operate autonomously
in natural environments. Humanoid robots, with their human-like physique, naturally fit into the
human world. With recent advances in hardware designs and increased commercial availability,
† This work was done while Jinhan Li was a visiting researcher at UT Austin.
* Equal contribution
8th Conference on Robot Learning (CoRL 2024), Munich, Germany.
humanoid robots emerge as a promising platform to deploy in our living and working spaces. Despite
their great potential, they still struggle to interact autonomously and robustly in the unstructured
world. A burgeoning line of work has resorted to deep imitation learning methods for humanoid
manipulation [1–3]. However, they rely on large amounts of demonstrations through whole-body
teleoperation, requiring domain expertise and strenuous efforts. In contrast, humans have the innate
ability to watch their peers do a task once and mimic. Equipping robots with such an imitation
ability will move us closer to the goal of learning from Internet-scale human activity videos.
We explore teaching humanoid robots to manipulate objects by watching humans. We consider a
problem setting recently formulated as “open-world imitation from observation,” where a robot im-
itates a manipulation skill from a single video of human demonstration [4–6]. This setting would
facilitate users in effortlessly demonstrating tasks by doing and enable a humanoid robot to acquire
new skills quickly. Enabling humanoids to imitate from single videos presents a significant chal-
lenge — the video does not have action labels, but yet the robot has to learn to perform tasks in
new situations beyond what’s demonstrated in the video. Prior works on one-shot video learning
have attempted to optimize robot actions to reconstruct the future object motion trajectories [4, 5].
However, they have been applied to single-arm manipulators and are computationally prohibitive
for humanoid robots due to their high degrees of freedom and joint redundancy [7]. Meanwhile,
the similar kinematic structure shared by humans and humanoids makes directly retargeting human
motions to robots feasible [8, 9]. Nonetheless, existing retargeting techniques focus on free-space
body motions [10–14], lacking the contextual awareness of objects and interactions needed for ma-
nipulation. To address this shortcoming, we introduce the concept of “object-aware retargeting.”
By incorporating object contextual information into the retargeting process, the resulting humanoid
motions can be efficiently adapted to the locations of objects in open-ended environments.
To this end, we introduce OKAMI (Object-aware Kinematic retArgeting for huManoid Imitation),
an object-aware retargeting method enables a bimanual humanoid with two dexterous hands to imi-
tate manipulation behaviors from a single RGB-D video demonstration. OKAMI uses a two-stage
process to retarget the human motions to the humanoid robot to accomplish the task across varying
initial conditions. The first stage processes the video to generate a reference manipulation plan.
The second stage uses this plan to synthesize the humanoid motions through motion retargeting that
adapts to the object locations in target environments.
OKAMI includes two key designs. The first design is an open-world vision pipeline that identi-
fies task-relevant objects, reconstructs human motions from the video, and localizes task-relevant
objects during evaluation. Localizing objects at test time also enables motion retargeting to adapt
to different backgrounds or new object instances of the same categories. The second design is the
factorized process for retargeting, where we retarget the body motions and hand poses separately.
We first retarget the body motions from the reference plan in the task space, and then warp the retar-
geted trajectory given the location of task-relevant objects. The trajectory of body joints is obtained
through inverse kinematics. The joint angles of fingers are mapped from the plan onto the dexterous
hands, reproducing hand-object interaction. With object-aware retargeting, OKAMI policies sys-
tematically generalize across various spatial layouts of objects and scene clutters. Finally, we train
visuomotor policies on the rollout trajectories from OKAMI through behavioral cloning to obtain
vision-based manipulation skills.
We evaluate OKAMI on human video demonstrations of diverse tasks that cover rich object inter-
actions, such as picking, placing, pushing, and pouring. We show that its object-aware retargeting
achieves 71.7%
by 58.3%
achieving an average success rate of 79.2%
1. OKAMI enables a humanoid robot to mimic human behaviors from a single video for
dexterous manipulation. Its object-aware retargeting process generates feasible motions of
the humanoid robot while adapting the motions to target object locations at test time;
2. OKAMI uses vision foundation models [15, 16] to identify task-relevant objects with-
out additional human inputs. Their common-sense reasoning ability helps recognize task-
2
relevant objects even if they are not directly in contact with other objects or the robot hands,
allowing our method to imitate more diverse tasks than prior work;
3. We validate OKAMI’s systematic generalization capabilities on real humanoid robot hard-
ware. OKAMI enables real-robot deployment in natural environments with varying visual
backgrounds, unseen object layouts, and new instances of task-relevant objects.
2 Related Work
Humanoid Robot Control. A large body of literature has studied controlling humanoid robots to
complete locomotion or manipulation tasks [10, 12, 17]. Methods like motion planning or optimal
control typically require a perfect physics model of the humanoid robot and are often computation-
ally expensive [11, 12, 18]. People have explored using the sim-to-real paradigm, where they train
reinforcement learning agents in simulation with domain randomization so that the policies can be
transferred robustly. However, such a method is typically limited by the simulation tasks that can be
created and often only limited to the locomotion tasks [10], whereas the simulation of manipulation
tasks is hard to design, not to mention the reward functions. Using human data makes humanoid
robot control easier, given the similar kinematic structures between humans and humanoids. The
control can be done through teleoperation, using either motion capture suits [9, 12, 19–23], telex-
istence cockpits [24–28], VR devices [1, 29, 30], or using RGB video to track human motion [17].
However, such remote control requires real-time control of human teleoperators, posing both great
mental and physical stress on the teleoperators. Instead, we focus on the setting where a robot
watches the human perform a manipulation task in an RGB-D video. While existing literature has
explored such an imitation setup in the scope of tabletop manipulation [4–6], we are the first to study
the problem within the scope of humanoid manipulation.
Learning From Demonstrations/Imitation Learning. Imitation Learning has progressed signifi-
cantly in learning vision-based robot manipulation with high sample efficiency [31–42]. Prior works
have shown that with dozens of demonstrations, a robot can learn a visuomotor policy that completes
various tasks, ranging from long-horizon manipulation tasks [32–34] to dexterous manipulation [35–
37]. However, collecting demonstrations often requires expertise in using teleoperation devices,
creating barriers to usability. Another line of work focuses on one-shot imitation learning [38, 39]
or imitating from a single demonstration [40–42]. However, they either require additional data col-
lection during a meta-training stage or still require teleoperation. Recently, people have shifted
their focus towards imitating a single video demonstration without ground-truth label [4–6]. This
problem was recently defined as “open-world imitation from observation” [4]. However, unlike
prior works that explicitly abstract away the embodiment motions due to the kinematic differences
between humans and robot arms, we exploit the embodiment information due to the embodiment
similarity between human bodies and humanoid robots. In this work, OKAMI focuses on what we
call object-aware retargeting. It is a method that adapts the motion of human bodies to humanoid
robots so that we can achieve humanoid robot imitation.
Motion Retargeting. Motion retargeting has been long studied for adapting the motion of a person
or a character to another character[8]. Retargeting has a wide application in computer graphics and
3D vision communities, where literature has extensively studied how to retarget human motions to
human digital avatars [43–45]. This technique has been extended to robotics, where researchers fo-
cus on how to reuse the motions of a human and recreate similar behaviors on a humanoid robot or
other robots with anthropomorphism. Rich liteartures have investigated how to do retargeting with
a variety of methodology, such as optimization-based (QP, motion planning, IK) [11, 12, 19, 46],
geometric-based (affine mapping, etc.) [47], and learning-based [10, 13, 17]. These methods have
been successfully used in generating quadruped locomotion, loco-manipulation, humanoid locomo-
tion, manipulation, and loco-manipulation. However, these retargeting methods have been used in
teleoperation systems in the scope of manipulation tasks, as they lack a vision pipeline that allows
the robot to adapt to object locations automatically. In this work, we connect the retargeting process
with open-world vision, endowing the retargeting process with object awareness so that the robot
mimics the human motions from a video demonstration and adapts to the object locations at test time.
3
3 OKAMI
In this work, we introduce OKAMI, a two-staged method that tackles “open-world imitation from
observation” [4]. OKAMI first generates a reference plan using the object locations and recon-
structed human motions from a given RGB-D video; then it retargets the human motions trajectories
to the humanoid robot while adapting the trajectories based on new locations of the objects. Figure 2
illustrates the whole pipeline.
3.1 Problem Formulation
We formulate a humanoid manipulation task as a discrete-time Markov Decision Process defined
by a tuple: M = (S, A, P, R, γ, μ), where S is the state space, A is the action space, P (·|s, a) is
the transition probability, R(s) is the reward function, γ ∈ [0, 1) is the discount factor, and μ is
the initial state distribution. In our context, S is the space of raw RGB-D observations that capture
both the robot and object states, A is the space of the motion commands for the humanoid robot,
R is the sparse reward function that returns 1 when a task is complete. The objective of solving a
task is to find a policy π that maximizes the expected task success rates from a wide range of initial
configurations drawn from μ at test time.
In this paper, we consider the setting of “open-world imitation from observation” [4], where the robot
system takes a recorded RGB-D human video, V as input, and returns a humanoid manipulation
policy π that completes the task as demonstrated in V . This setting is “open-world” as the robot
does not have prior knowledge or ground-truth access to the categories or physical states of objects
involved in the task, and it is “from observation” in the sense that video V does not come with any
ground-truth robot actions. A policy execution is considered successful if the state matches the states
of the final frame from V . The success conditions of al tested tasks are described in Appendix B.1.
Notably, two assumptions are made about V in this paper: all the image frames in V capture the
human bodies, and the camera view of shooting V is static throughout the recording.
3.2 Reference Plan Generation
To enable object-aware retargeting, OKAMI first needs to generate a reference plan for the hu-
manoid robot to follow. Here, we describe how the reference plan is generated. To this end, OKAMI
needs to understand what objects are involved and how humans move the objects in the demonstrated
task, which are described first before we introduce the plan generation step.
Identify and Localize Task-Relevant Objects. Imitating a manipulation task requires the robot
to understand what objects to interact with in order to complete the task. However, identifying task-
relevant objects from pure images is a nontrivial challenge. While prior works use unsupervised
approach to identify the objects [48, 49], they often assume simple visual backgrounds. Other al-
ternatives require additional linguistic inputs from humans, inducing extra annotation cost from the
user [50, 51]. Instead, we observe that most objects in everyday tasks are covered by common sense
knowledge, where state-of-the-art Vision-Language Models (VLMs) such as GPT4V have internal-
ized such knowledge through pre-training on internet data. Based on such observation, we leverage
the power of GPT4V to identify task-relevant objects directly from the video demonstration V . Con-
cretely, OKAMI samples the RGB image frames from V and prompting GPT4V with the concate-
nated image of the sampled frames (Appendix A.2 describe the details of test prompt we use to query
the object names from GPT4V). GPT4V returns a list of texts that describe the names of task-relevant
objects in V . Subsequently, OKAMI uses Grounded-SAM [16] with the list of object names to seg-
ments the objects on the first frame of V , and then track their locations across the entire video
by propagating the first frame segmentation throughout the images using Cutie [52]. In the end,
OKAMI localizes the task-relevant objects in V , which is the cornerstone for all subsequent steps.
Reconstruct Human Motions. As mentioned in Section 1, retargeting human motions to the
humanoid has great potential to generate feasible actions for humanoids due to their human-like
embodiments. However, the video demonstration V does not come with annotations on the hu-
4
SMPL-H trajectory
segment
Inverse
Kinematics
Hand Finger
Mapping
Return a list of task-
relevant object names
“bottle”
“bowl”
GPT4V
RGB-D Video
Retarget motions
Using SMPL-H Warped motions
<latexit sha1_base64="L8wFmirgYiqIexNq3ulkzL02sEI=">AAAB7HicbVBNS8NAEJ3Ur1q/qh69LBbBU0lE1GPRi8cKpi20oWy2m3bpZhN2J0IJ/Q1ePCji1R/kzX/jts1BWx8MPN6bYWZemEph0HW/ndLa+sbmVnm7srO7t39QPTxqmSTTjPsskYnuhNRwKRT3UaDknVRzGoeSt8Px3cxvP3FtRKIecZLyIKZDJSLBKFrJl/3cnfarNbfuzkFWiVeQGhRo9qtfvUHCspgrZJIa0/XcFIOcahRM8mmllxmeUjamQ961VNGYmyCfHzslZ1YZkCjRthSSufp7IqexMZM4tJ0xxZFZ9mbif143w+gmyIVKM+SKLRZFmSSYkNnnZCA0ZygnllCmhb2VsBHVlKHNp2JD8JZfXiWti7p3Vb98uKw1bos4ynACp3AOHlxDA+6hCT4wEPAMr/DmKOfFeXc+Fq0lp5g5hj9wPn8Av0+OqA==</latexit>
l0
<latexit sha1_base64="9L/YXDXQXOLHv1NEoN5OIoOdPBM=">AAAB7HicbVBNS8NAEJ3Ur1q/qh69LBbBU0lE1GPRi8cKpi20oWy2m3bpZhN2J0IJ/Q1ePCji1R/kzX/jts1BWx8MPN6bYWZemEph0HW/ndLa+sbmVnm7srO7t39QPTxqmSTTjPsskYnuhNRwKRT3UaDknVRzGoeSt8Px3cxvP3FtRKIecZLyIKZDJSLBKFrJl/3cm/arNbfuzkFWiVeQGhRo9qtfvUHCspgrZJIa0/XcFIOcahRM8mmllxmeUjamQ961VNGYmyCfHzslZ1YZkCjRthSSufp7IqexMZM4tJ0xxZFZ9mbif143w+gmyIVKM+SKLRZFmSSYkNnnZCA0ZygnllCmhb2VsBHVlKHNp2JD8JZfXiWti7p3Vb98uKw1bos4ynACp3AOHlxDA+6hCT4wEPAMr/DmKOfFeXc+Fq0lp5g5hj9wPn8AwNSOqQ==</latexit>
l1
<latexit sha1_base64="jAfvAxTKmAyIZRV+BmWd/JpcKvI=">AAAB7HicbVBNS8NAEJ3Ur1q/qh69LBbBU0mkqMeiF09SwbSFNpTNdtsu3WzC7kQoob/BiwdFvPqDvPlv3LY5aOuDgcd7M8zMCxMpDLrut1NYW9/Y3Cpul3Z29/YPyodHTROnmnGfxTLW7ZAaLoXiPgqUvJ1oTqNQ8lY4vp35rSeujYjVI04SHkR0qMRAMIpW8mUvu5/2yhW36s5BVomXkwrkaPTKX91+zNKIK2SSGtPx3ASDjGoUTPJpqZsanlA2pkPesVTRiJsgmx87JWdW6ZNBrG0pJHP190RGI2MmUWg7I4ojs+zNxP+8ToqD6yATKkmRK7ZYNEglwZjMPid9oTlDObGEMi3srYSNqKYMbT4lG4K3/PIqaV5Uvctq7aFWqd/kcRThBE7hHDy4gjrcQQN8YCDgGV7hzVHOi/PufCxaC04+cwx/4Hz+AOzljsY=</latexit>
lN
Reference Plan
SMPL-H trajectory
Track objects across
the video
Identify Keyframes Through
Changepoint Detections
Human
Reconstruction
Model <latexit sha1_base64="L8wFmirgYiqIexNq3ulkzL02sEI=">AAAB7HicbVBNS8NAEJ3Ur1q/qh69LBbBU0lE1GPRi8cKpi20oWy2m3bpZhN2J0IJ/Q1ePCji1R/kzX/jts1BWx8MPN6bYWZemEph0HW/ndLa+sbmVnm7srO7t39QPTxqmSTTjPsskYnuhNRwKRT3UaDknVRzGoeSt8Px3cxvP3FtRKIecZLyIKZDJSLBKFrJl/3cnfarNbfuzkFWiVeQGhRo9qtfvUHCspgrZJIa0/XcFIOcahRM8mmllxmeUjamQ961VNGYmyCfHzslZ1YZkCjRthSSufp7IqexMZM4tJ0xxZFZ9mbif143w+gmyIVKM+SKLRZFmSSYkNnnZCA0ZygnllCmhb2VsBHVlKHNp2JD8JZfXiWti7p3Vb98uKw1bos4ynACp3AOHlxDA+6hCT4wEPAMr/DmKOfFeXc+Fq0lp5g5hj9wPn8Av0+OqA==</latexit>
l0
<latexit sha1_base64="9L/YXDXQXOLHv1NEoN5OIoOdPBM=">AAAB7HicbVBNS8NAEJ3Ur1q/qh69LBbBU0lE1GPRi8cKpi20oWy2m3bpZhN2J0IJ/Q1ePCji1R/kzX/jts1BWx8MPN6bYWZemEph0HW/ndLa+sbmVnm7srO7t39QPTxqmSTTjPsskYnuhNRwKRT3UaDknVRzGoeSt8Px3cxvP3FtRKIecZLyIKZDJSLBKFrJl/3cm/arNbfuzkFWiVeQGhRo9qtfvUHCspgrZJIa0/XcFIOcahRM8mmllxmeUjamQ961VNGYmyCfHzslZ1YZkCjRthSSufp7IqexMZM4tJ0xxZFZ9mbif143w+gmyIVKM+SKLRZFmSSYkNnnZCA0ZygnllCmhb2VsBHVlKHNp2JD8JZfXiWti7p3Vb98uKw1bos4ynACp3AOHlxDA+6hCT4wEPAMr/DmKOfFeXc+Fq0lp5g5hj9wPn8AwNSOqQ==</latexit>
l1
<latexit sha1_base64="jAfvAxTKmAyIZRV+BmWd/JpcKvI=">AAAB7HicbVBNS8NAEJ3Ur1q/qh69LBbBU0mkqMeiF09SwbSFNpTNdtsu3WzC7kQoob/BiwdFvPqDvPlv3LY5aOuDgcd7M8zMCxMpDLrut1NYW9/Y3Cpul3Z29/YPyodHTROnmnGfxTLW7ZAaLoXiPgqUvJ1oTqNQ8lY4vp35rSeujYjVI04SHkR0qMRAMIpW8mUvu5/2yhW36s5BVomXkwrkaPTKX91+zNKIK2SSGtPx3ASDjGoUTPJpqZsanlA2pkPesVTRiJsgmx87JWdW6ZNBrG0pJHP190RGI2MmUWg7I4ojs+zNxP+8ToqD6yATKkmRK7ZYNEglwZjMPid9oTlDObGEMi3srYSNqKYMbT4lG4K3/PIqaV5Uvctq7aFWqd/kcRThBE7hHDy4gjrcQQN8YCDgGV7hzVHOi/PufCxaC04+cwx/4Hz+AOzljsY=</latexit>
lN
Identify target / ref objects and
generate reference plan
Reference Plan
Generation
Target and
reference objects
Object-Aware
Retargeting
Localize relevant objects
at test time
Robot Observation
Reference Plan
Send Joint
Commands
Estimate transformation
between point clouds
Robot executionFigure 2: Overview of OKAMI. OKAMI is a two-staged method that enables a humanoid robot to imitate
a manipulation task from a single human video. In the first stage, OKAMI generates a reference plan for
subsequent manipulation, and the plan generation process uses GPT4V and multiple large vision models. In
the second stage, OKAMI follows the reference plan, where it retargets human motions onto the humanoid with
object awareness for each step of the plan. The retargeted motions are converted into robot joint configurations,
and the humanoid robot follows the joint configurations to complete the demonstrated manipulation task.
man motions. To annotate videos with human motions, we adopt SLAHMR [53], an iterative op-
timization algorithm that models the sequence of human motions from videos. SLAHMR models
the human motions by minimizing the error between the 2D projection of 3D joints from human
meshes, SMPL (Skinned Multi-Person Linear Model) models [54], and the detected 2D joint loca-
tions of human poses [53]. The initial SMPL models are initialized by using an off-the-shelf model
PHALP [55], which directly predicts the parameters of SMPL from videos. However, SLAHMR
only models the body poses and assumes flat hands in the videos, while mapping human motions
to a humanoid robot demands both body and hand poses for manipulation. To address the limita-
tion, we introduce the following design that improves the original SLAHMR: we use the SMPL+H
model [56], an extended representation of SMPL that includes hand poses, and we initialize the pose
of the hands in every frame using 3D hand estimates from HaMeR [57]. Then we use the joint op-
timization from SLAHMR to optimize over SMPL+H models instead of SMPL models to finetune
the body location, body poses, and hand poses over the video (Full details about the process are
provided in Appendix A.1).
The modified SLAHMR outputs a sequence of SMPL-H, which capture the human body and hand
poses throughout the video. From the trajectory of SMPL-H models, we obtain the estimated full-
body poses, which include locations of body joints in the task space with respect to the human
pelvis, and hand poses in joint configurations that describe how a hand interacts with an object.
With the SMPL-H trajectories, OKAMI is able to retarget the human motions to the humanoids,
which will be explained in Section 3.3. One advantage of using SMPL-H representation is that it
captures human body poses while being invariant across humans with different demographics, and
SMPL-H representation is easy to retarget motions to the humanoid robot that has different sizes
from the human. As our experiments show, OKAMI is able to handle variations across different
demonstrations.
Generate a Plan From V . From the previous two steps, the robot has the notion of both task-
relevant objects and how human manipulate the objects. However, naively warping the entire human
motion trajectory based on object locations doom to fail. Instead, OKAMI needs to identify the
5
subgoals in V such that we can warp segment of trajectories conditioning on the location of the
object that is associated with a subgoal.
We first identify subgoals by performing temporal segmentation on the video sequence. The tempo-
ral segmentation is performed as follows: We sample keypoints within the first frame segmentation
and use an off-the-shelf Tracky-Any-Point model, CoTracker [58], to track the keypoints in the
video. Given these tracked keypoint trajectories, we compute the average velocity of keypoints at
each frame, and use a standard unsupervised changepoint detection algorithm [59] to detect the large
changes in the velocity statistics. The changepoint detection returns a list of keyframes as a result,
where each keyframe in the video corresponds to a subgoal state.
Next, we identify a target object (the object in motion due to manipulation) and a reference object
(the object that serves as a spatial reference for the target object’s movements through either contact
or non-contact relations) for achieving each subgoal. The target object is determined by computing
the average velocity per object using the average velocities of keypoints, and the reference object is
subsequently determined if an object has either contact or non-contact relations with the target ob-
ject. Whether two objects are in contact or not is decided based on a geometric heuristic, computing
their relative spatial locations and the distances between point clouds of objects. As for non-contact
relations, such as the target cup in a pouring task, which might never be touched by a hand or the
kettle, it is inherently ambiguous to determine such relations through general geometric heuristics
such as distance. Instead, we use GPT4V, which has the common-sense knowledge to predict the
semantic relations between objects.
Once the subgoals and associated objects are determined, we generate a reference plan, represented
as {l0, l1, . . . , lN }, where each step li corresponds to an identified keyframe. Each step stores a
three-element tuple (otarget, oreference, τ SMPL
ti:ti+1 ), which are the point clouds of the target object, the
reference object and the SMPL-H trajectory segment between two keyframes, respectively. Note
that oreference can be null if there is no spatial reference required for a step (e.g., grasping an object
or closing a drawer as opposed the placing, where reference object is required). All the point clouds
are obtained by back-projecting the segmented objects from RGB images using depth images [60].
3.3 Object-Aware Retargeting
Given a reference plan generated from the video demonstration, the humanoid robot follows the
plan to imitate the demonstrated task in V . The robot follows each step li in the plan, where it first
localizes the task-relevant objects, and retargets the corresponding segment of SMPL-H trajectory
onto the humanoid while taking into account the target and reference objects. Then the retargeted
trajectories are converted to the joint configuration trajectory using inverse kinematics for the robot
hardware to execute. This process repeats until all the steps are executed and we evaluate if a rollout
is successful or not following the success conditions of each task, as explained in Appendix B.1.
Localize Objects at Test Time. The reference plan is executed step by step, with each step contain-
ing a tuple of information about the target object, reference object, and the corresponding subgoal-
bounded SMPL-H trajectory. To adapt the plan to the test-time environment, we localize the objects
specified in the tuple using the robot’s current observation. By extracting 3D point clouds of the
objects from the robot’s perception system, we can accurately track their positions and orientations.
Localizing the objects at test-time paves the way for OKAMI to achieve systematic generaliza-
tion across various visual conditions, including different backgrounds, and with new instances of
task-relevant objects.
Retarget Human Motions to the Humanoid. The key aspect of object-awareness in our approach
is the ability to adapt to new locations of objects. Once OKAMI localizes the objects in the observa-
tion, we develop a retargeting process that adapts humanoid motions to the object locations. Specif-
ically, we employ a factorized process that separates the retargeting of the arm and hand motions. In
this process, OKAMI first adapts the arm motions to the object locations so that the fingers of the
hands are placed within the object-centric coordinate frame. Then OKAMI only needs to retarget
fingers in the joint configuration to mimic how the human interacts with objects with their hands.
6
Sprinkle-salt Plush-toy-in-basket Close-the-laptop
Close-the-drawer Place-snacks-on-plate BaggingFigure 3: Visualization of initial and final frames of both human demonstrations and robot rollouts for all tasks.
Concretely, the retargeting process begins by mapping the human body motions from the task space
to the humanoid robot. This process involves scaling and adjusting the trajectories to account for
the differences in size and proportion between the human and the robot. Next, OKAMI warps
the retargeted trajectory based on the locations of the objects observed at test time. Intuitively,
the warping step “bends” the trajectory to ensure that the robot’s arm reaches the objects in their
new positions while maintaining the overall trajectory shape of the demonstrated motions, making
humanoid motions look natural. We warp the retargeted trajectory following the practice as in prior
work [4], which adapts the trajectory to object locations at test time that are different from the ones
seen in videos, while retaining the curvature and direction of the trajectory from starting point to
the end point (More details in Appendix A.4). Specifically, there are two cases we consider for
warping the trajectory: the first case is when there are no changes to the relational state between the
target and the reference object or no reference object exists. In that case, we only warp the trajectory
conditioning on the locations of the target object; the second case is where the relation state changes,
meaning the trajectory needs to be conditioned on the reference object location.
Once the arm trajectory is warped, we use inverse kinematics to solve a sequence of joint configu-
rations for the arms. For positions and rotation, we assigned weights of 1.0 and 0.08 for position
and rotation of hands respectively so that the robot hand reaches desired locations while the arms
maintain natural postures. At the same time, we retarget the human’s hand poses to the robot in the
configuration space. This means that we map the joint angles of the human hand to the corresponding
joint angles of the robot’s hand, ensuring that the robot can replicate the fine-grained manipulations
demonstrated by the human. Implementation details are provided in Appendix A.3. Together, we
have the trajectory of full-body joint configurations for the real robot hardware to execute using a
low-level robot controller.
Since the retargeting of arm motions between the human and the humanoid is affine, the retargeting
process naturally allows us to scale and adjust motions given demonstrators with different demo-
graphics such as heights. By adapting the arm trajectories to the object locations and retargeting the
hand poses independently, OKAMI’s factorized process of retargeting achieves systematic general-
ization across various spatial layouts.
7
Success rate Missed grasping Failed Completion
75.0%
Place-snacks-
on-plate
75.0%
58.3%
66.7%
Demonstrator 1 Demonstrator 2 Demonstrator 3
75.0%
83.3%
75.0%
58.3%
Sprinkle-salt
66.7%
Plush-toy-in-
basket
83.3%
Close-the-
laptop
75.0%
Close-the-
drawer
Place-snacks-
on-plate
Close-the-
laptop
(a) (b)
58.3%
BaggingFigure 4: (a) Evaluation of OKAMI over all six tasks, including the success rates and the quantification of
failed trials, separated by failure mode. (b) Evaluation of OKAMI using videos from different demonstrations.
Demonstrator 1 is the main person recording videos for all evaluations in (a).
4 Experiments
Our experiments are designed to answer the following research question: 1) Is OKAMI effective for
a humanoid robot to imitate diverse manipulation tasks by watching single videos of human demon-
strations? 2) Is it critical in OKAMI to retarget the body motions of demonstrators to the humanoid
robot instead of only retargeting based on object locations? 3) Does OKAMI keep the good perfor-
mance consistently given videos of the same task demonstrated by users with diverse demographics?
4) Are the rollouts generated by OKAMI effective for training closed-loop visuomotor policies?
4.1 Experimental Setup
Tasks. Here we describe the tasks we choose. 1) Plush-toy-in-basket: placing
a plush toy in the basket; 2) Sprinkle-salt: sprinkling a bit of salt into the bowl; 3)
Close-the-drawer: pushing the drawer in to close it; 4) Close-the-laptop: closing
the lid of the laptop; 5) Place-snacks-on-plate: placing a bag of snacks on the plate. 6)
Bagging: placing a chip bag into to a shopping bag. We select these six tasks that cover all
kinds of manipulation behaviors: Plush-toy-in-basket and Place-snacks-on-plate
require pick-and-place behaviors of daily objects; Sprinkle-salt is the task that covers pour-
ing behavior; Close-the-drawer and Close-the-laptop require the humanoid to interact
with articulated objects, which is a common interaction exist in daily environments; Bagging is
the task that involves bimanual interaction and includes multiple subgoals. While we mainly focus
on real robot experiments, we also implement Sprinkle-salt and Close-the-drawer in
simulation using Robosuite [61] for easy reproducibility of OKAMI. See Appendix B.4.
Hardware Setup. We use Fourier-GR1 as the real robot hardware evaluation. The robot is equipped
with two 6-DoF Inspire dexterous hands. For both video recording and robot camera observation,
we use the D435i Intel RealSense camera. In all our experiments, we use a joint position controller
that operates at 400Hz. To avoid jerky movements, we command the joint position targets at 40Hz
and interpolate the commands to 400Hz trajectories.
Evaluation Protocol. We evaluate 12 trials for each task. The locations of the objects are
initialized within the intersection of the robot camera’s view and the humanoid arms’ reachable
range. The tasks are evaluated on a tabletop workspace with multiple objects, including both
task-relevant objects and various other objects. Further, we test new object generalization on
Place-snacks-on-plate, Plush-toy-in-basket, and Sprinkle-salt tasks, chang-
ing the involved plate, snack bag, plush toy, and bowl to other instances of the same type.
Baselines. We compare our result with a baseline ORION [4]. Since ORION was proposed for
parallel-jaw grippers, we cannot directly apply it in our experiments. To evaluate ORION in the hu-
manoid experiments, we’ve made minimal modifications: we estimate the palm trajectory using the
SMPL-H trajectories, and warp the trajectory conditioning on the new object locations. The warped
trajectory is used in the subsequent inverse kinematics for computing robot joint configurations.
8
4.2 Quantitative Results
To answer question (1), we evaluate the policies of our method across six different tasks (introduced
in the experimental setup section), which cover diverse behaviors such as daily pick-place, pouring,
and manipulation of articulated objects. The result is shown in Figure 4(a). In our experiment,
we randomly initialize the object locations, so that the robot needs to adapt to the locations of
the objects. This result supports the design of OKAMI and shows its effectiveness in achieving
systematic generalizations over different visual and spatial conditions.
To answer question (2), we compare OKAMI against ORION on two representative tasks,
Place-snacks-on-plate and Close-the-laptop. In the comparison experiment,
OKAMI differs from ORION in that ORION does not condition on the human body poses.
OKAMI achieves 75.0%
and 41.2%
versions of Sprinkle-salt and Close-the-drawer tasks. In simulation, OKAMI achieves
82.0%
tively. Most failures of ORION policies are due to failing to approach objects with reliable grasping
poses (e.g. in Place-snacks-on-plate task, ORION tries to grasp the snack from the sides
instead of the top-down grasp in human video), and failing to rotate the wrist fully to achieve behav-
iors such as pouring. These behaviors originate from the fact that ORION ignores the embodiment
information, thus falling short in performance compared to OKAMI. The outperforming result sug-
gests the importance of retargeting the body motion of the human demonstrators onto the humanoid
when imitating from human videos.
To answer question (3), we conduct a controlled experiment of recording videos of different demon-
strators and test if OKAMI policies maintain good performance across different video inputs.
Same as the previous experiment, we evaluate OKAMI on Place-snacks-on-plate and
Close-the-laptop task. The result is shown in Figure 4(b). We show that for the task
Close-the-laptop, there is no statistical significance in performance change. As for task
Place-snacks-on-plate, while the evaluation maintains above 50%
formance is 16.7%
we find that the motion of demonstrator 2 is relatively faster than the other two demonstrators, and
faster motions create noisy estimation of motion when doing human model reconstruction. Overall,
OKAMI is able to maintain reasonably good performance given videos from different demonstra-
tors, but there is room for improvements to handle such variety.
4.3 Learning Visuomotor Policy With OKAMI Rollout Data
OKAMI is an open-loop policy that does not respond to visual observations reactively. We also aim
to train closed-loop visuomotor policies that allow humanoid robots to respond to visual observa-
tions in real-time. We answer the question (4) by training neural-network-based visuomotor policies
with OKAMI rollouts.
We first evaluate OKAMI over randomly initialized object layouts, generating a number of rollout
trajectories. Then, we collect the successful rollouts by filtering out the failed ones. Subsequently,
we use a behavioral cloning algorithm to train neural-network-based visuomotor policies. As smooth
execution is critical when a humanoid robot performs the manipulation, we implement the behavioral
cloning algorithm with ACT [62], which predicts smooth actions over its temporal ensemble design,
a trajectory smoothing component. More details are described in Appendix B.5.58.3%
50 Trajectories 100 Trajectories
75.0%
Using the behavioral cloning algorithm, we ef-
fectively distill the successful rollout data gen-
erated by OKAMI into a neural network that
operationalizes closed-loop visuomotor poli-
cies on humanoid manipulation tasks.
9
We train visuomotor policies for
Sprinkle-salt and Bagging. Fig-
ure 5 visualizes the success rates of the
policies, showing that OKAMI rollouts are ef-
fective data sources for training policies. Also,
we show that the learned visuomotor policies
improve as more rollouts are collected. These
results hold the promise of scaling up data
collection for learning humanoid manipulation
skills without laborious teleoperation.
5 Conclusion
This paper introduces OKAMI that enables a humanoid robot to imitate a single RGB-D human
video demonstration. At the core of OKAMI is object-aware retargeting, which retargets the human
motions onto the humanoid robot and adapts the motions to the object locations. OKAMI consists
of two stages to realize object-aware retargeting. The first stage is generating a reference plan for
manipulation from the video. The second stage is used for retargeting, where OKAMI retargets
the arm motions in the task space and the finger motions in the joint configuration space. Our
experiments validate the design of OKAMI, showing the systematic generalization of OKAMI
policies. Additionally, OKAMI enables easy collection of rollout data starting with a single human
video demonstration. OKAMI-based data collection significantly reduces human effort compared
to that required by teleoperation.
Limitations. The focus of OKAMI is on the upper body motion retargeting of humanoid robots,
particularly for manipulation tasks within tabletop workspaces. A promising future direction is to
include lower body retargeting that enable locomotion behaviors during video imtiation. To enable
full-body loco-manipulation, whole-body motion controller needs to be imnplemented as oppposed
to the joint position controller we used in OKAMI.
Additionally, we focus on using RGB-D data in OKAMI, which prevents us from using in-the-wild
internet videos recorded in RGB. Extending OKAMI to use RGB videos will be another promising
direction for future works.
Also, the current implementation of retargeting has limited robustness against large variations in
object shapes. A future improvement would be integrating more powerful foundation models that
endow the robot with general understanding of how to interact with a class of objects in spite of their
large shape changes.
10
Acknowledgments
We would like to thank William Yue for providing the initial implementation of the behavioral
cloning policies, Peter Stone for his valuable support with task designs and demo shooting, Yuzhe
Qin for sharing the dex-retargeting codebase, and Zhenjia Xu for his advice in developing the hu-
manoid robot infrastructure.
References
[1] M. Seo, S. Han, K. Sim, S. H. Bang, C. Gonzalez, L. Sentis, and Y. Zhu. Deep imitation learn-
ing for humanoid loco-manipulation through human teleoperation. In IEEE-RAS International
Conference on Humanoid Robots (Humanoids), 2023.
[2] Y. Matsuura, K. Kawaharazuka, N. Hiraoka, K. Kojima, K. Okada, and M. Inaba. Development
of a whole-body work imitation learning system by a biped and bi-armed humanoid. In 2023
IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS), pages 10374–
10381. IEEE, 2023.
[3] T. Asfour, P. Azad, F. Gyarfas, and R. Dillmann. Imitation learning of dual-arm manipulation
tasks in humanoid robots. International journal of humanoid robotics, 5(02):183–202, 2008.
[4] Y. Zhu, A. Lim, P. Stone, and Y. Zhu. Vision-based manipulation from single human video
with open-world object graphs. arXiv preprint arXiv:2405.20321, 2024.
[5] N. Heppert, M. Argus, T. Welschehold, T. Brox, and A. Valada. Ditto: Demonstration imitation
by trajectory transformation. arXiv preprint arXiv:2403.15203, 2024.
[6] D. Guo. Learning multi-step manipulation tasks from a single human demonstration. arXiv
preprint arXiv:2312.15346, 2023.
[7] T. Asfour and R. Dillmann. Human-like motion of a humanoid robot arm based on a closed-
form solution of the inverse kinematics problem. In Proceedings 2003 IEEE/RSJ International
Conference on Intelligent Robots and Systems (IROS 2003)(Cat. No. 03CH37453), volume 2,
pages 1407–1412. IEEE, 2003.
[8] M. Gleicher. Retargetting motion to new characters. Proceedings of the 25th annual conference
on Computer graphics and interactive techniques, 1998.
[9] K. Darvish, Y. Tirupachuri, G. Romualdi, L. Rapetti, D. Ferigo, F. J. A. Chavez, and D. Pucci.
Whole-body geometric retargeting for humanoid robots. In 2019 IEEE-RAS 19th International
Conference on Humanoid Robots (Humanoids), pages 679–686. IEEE, 2019.
[10] X. Cheng, Y. Ji, J. Chen, R. Yang, G. Yang, and X. Wang. Expressive whole-body control for
humanoid robots. arXiv preprint arXiv:2402.16796, 2024.
[11] S. Nakaoka, A. Nakazawa, F. Kanehiro, K. Kaneko, M. Morisawa, and K. Ikeuchi. Task model
of lower body motion for a biped humanoid robot to imitate human dances. In 2005 IEEE/RSJ
International Conference on Intelligent Robots and Systems, pages 3157–3162. IEEE, 2005.
[12] K. Hu, C. Ott, and D. Lee. Online human walking imitation in task and joint space based on
quadratic programming. In 2014 IEEE International Conference on Robotics and Automation
(ICRA), pages 3458–3464. IEEE, 2014.
[13] S. Choi, M. K. Pan, and J. Kim. Nonparametric motion retargeting for humanoid robots on
shared latent space. In Robotics: Science and Systems, 2020.
[14] E. Demircan, T. Besier, S. Menon, and O. Khatib. Human motion reconstruction and synthesis
of human skills. In Advances in Robot Kinematics: Motion in Man and Machine: Motion in
Man and Machine, pages 283–292. Springer, 2010.
11
[15] OpenAI. Gpt-4 technical report, 2023.
[16] S. Liu, Z. Zeng, T. Ren, F. Li, H. Zhang, J. Yang, C. Li, J. Yang, H. Su, J. Zhu, et al. Grounding
dino: Marrying dino with grounded pre-training for open-set object detection. arXiv preprint
arXiv:2303.05499, 2023.
[17] T. He, Z. Luo, W. Xiao, C. Zhang, K. Kitani, C. Liu, and G. Shi. Learning human-to-humanoid
real-time whole-body teleoperation. In arXiv, 2024.
[18] A. Escande, N. Mansard, and P.-B. Wieber. Hierarchical quadratic programming: Fast online
humanoid-robot motion generation. The International Journal of Robotics Research, 33(7):
1006–1028, 2014.
[19] L. Penco, N. Scianca, V. Modugno, L. Lanari, G. Oriolo, and S. Ivaldi. A multimode teleop-
eration framework for humanoid loco-manipulation: An application for the icub robot. IEEE
Robotics & Automation Magazine, 26(4):73–82, 2019.
[20] D. Kim, B.-J. You, and S.-R. Oh. Whole body motion control framework for arbitrarily and
simultaneously assigned upper-body tasks and walking motion. Modeling, Simulation and
Optimization of Bipedal Walking, pages 87–98, 2013.
[21] A. Di Fava, K. Bouyarmane, K. Chappellet, E. Ruffaldi, and A. Kheddar. Multi-contact motion
retargeting from human to humanoid robot. In 2016 IEEE-RAS 16th international conference
on humanoid robots (humanoids), pages 1081–1086. IEEE, 2016.
[22] M. Arduengo, A. Arduengo, A. Colom´e, J. Lobo-Prat, and C. Torras. Human to robot whole-
body motion transfer. In 2020 IEEE-RAS 20th International Conference on Humanoid Robots
(Humanoids), pages 299–305. IEEE, 2021.
[23] R. Cisneros, M. Benallegue, K. Kaneko, H. Kaminaga, G. Caron, A. Tanguy, R. Singh, L. Sun,
A. Dallard, C. Fournier, et al. Team janus humanoid avatar: A cybernetic avatar to embody
human telepresence. In Toward Robot Avatars: Perspectives on the ANA Avatar XPRIZE
Competition, RSS Workshop, volume 3, 2022.
[24] S. Tachi, K. Komoriya, K. Sawada, T. Nishiyama, T. Itoko, M. Kobayashi, and K. Inoue.
Telexistence cockpit for humanoid robot control. Advanced Robotics, 17(3):199–217, 2003.
[25] J. Ramos and S. Kim. Humanoid dynamic synchronization through whole-body bilateral feed-
back teleoperation. IEEE Transactions on Robotics, 34(4):953–965, 2018.
[26] Y. Ishiguro, T. Makabe, Y. Nagamatsu, Y. Kojio, K. Kojima, F. Sugai, Y. Kakiuchi, K. Okada,
and M. Inaba. Bilateral humanoid teleoperation system using whole-body exoskeleton cockpit
tablis. IEEE Robotics and Automation Letters, 5(4):6419–6426, 2020.
[27] F. Abi-Farrajl, B. Henze, A. Werner, M. Panzirsch, C. Ott, and M. A. Roa. Humanoid teleoper-
ation using task-relevant haptic feedback. In 2018 IEEE/RSJ International Conference on Intel-
ligent Robots and Systems (IROS), pages 5010–5017, 2018. doi:10.1109/IROS.2018.8593521.
[28] M. Schwarz, C. Lenz, A. Rochow, M. Schreiber, and S. Behnke. Nimbro avatar: Interactive
immersive telepresence with force-feedback telemanipulation. In 2021 IEEE/RSJ International
Conference on Intelligent Robots and Systems (IROS), pages 5312–5319. IEEE, 2021.
[29] M. Hirschmanner, C. Tsiourti, T. Patten, and M. Vincze. Virtual reality teleoperation of a
humanoid robot using markerless human upper body pose imitation. in 2019 ieee-ras 19th
international conference on humanoid robots (humanoids), 2019.
[30] D. Lim, D. Kim, and J. Park. Online telemanipulation framework on humanoid for both manip-
ulation and imitation. 2022 19th International Conference on Ubiquitous Robots (UR), pages
8–15, 2022. URL https://api.semanticscholar.org/CorpusID:250577582.
12
[31] A. Mandlekar, D. Xu, J. Wong, S. Nasiriany, C. Wang, R. Kulkarni, L. Fei-Fei, S. Savarese,
Y. Zhu, and R. Mart´ın-Mart´ın. What matters in learning from offline human demonstrations
for robot manipulation. arXiv preprint arXiv:2108.03298, 2021.
[32] A. Mandlekar, D. Xu, R. Mart´ın-Mart´ın, S. Savarese, and L. Fei-Fei. Learning to general-
ize across long-horizon tasks from human demonstrations. arXiv preprint arXiv:2003.06085,
2020.
[33] C. Wang, L. Fan, J. Sun, R. Zhang, L. Fei-Fei, D. Xu, Y. Zhu, and A. Anandkumar. Mimicplay:
Long-horizon imitation learning by watching human play. arXiv preprint arXiv:2302.12422,
2023.
[34] Y. Zhu, A. Joshi, P. Stone, and Y. Zhu. Viola: Imitation learning for vision-based manipulation
with object proposal priors. arXiv preprint arXiv:2210.11339, 2022.
[35] C. Wang, H. Shi, W. Wang, R. Zhang, L. Fei-Fei, and C. K. Liu. Dexcap: Scalable and portable
mocap data collection system for dexterous manipulation. arXiv preprint arXiv:2403.07788,
2024.
[36] T. Lin, Y. Zhang, Q. Li, H. Qi, B. Yi, S. Levine, and J. Malik. Learning visuotactile skills with
two multifingered hands. arXiv preprint arXiv:2404.16823, 2024.
[37] Y. Ze, G. Zhang, K. Zhang, C. Hu, M. Wang, and H. Xu. 3d diffusion policy. arXiv preprint
arXiv:2403.03954, 2024.
[38] M. Chang and S. Gupta. One-shot visual imitation via attributed waypoints and demonstration
augmentation. arXiv preprint arXiv:2302.04856, 2023.
[39] T. Yu, P. Abbeel, S. Levine, and C. Finn. One-shot composition of vision-based skills from
demonstration. In 2019 IEEE/RSJ International Conference on Intelligent Robots and Systems
(IROS), pages 2643–2650. IEEE, 2019.
[40] E. Valassakis, G. Papagiannis, N. Di Palo, and E. Johns. Demonstrate once, imitate imme-
diately (dome): Learning visual servoing for one-shot imitation learning. In 2022 IEEE/RSJ
International Conference on Intelligent Robots and Systems (IROS), pages 8614–8621. IEEE,
2022.
[41] E. Johns. Coarse-to-fine imitation learning: Robot manipulation from a single demonstration.
In 2021 IEEE international conference on robotics and automation (ICRA), pages 4613–4619.
IEEE, 2021.
[42] N. Di Palo and E. Johns. Learning multi-stage tasks with one demonstration via self-replay. In
Conference on Robot Learning, pages 1180–1189. PMLR, 2022.
[43] Z. Luo, J. Cao, K. Kitani, W. Xu, et al. Perpetual humanoid control for real-time simulated
avatars. In Proceedings of the IEEE/CVF International Conference on Computer Vision, pages
10895–10904, 2023.
[44] X. B. Peng, Z. Ma, P. Abbeel, S. Levine, and A. Kanazawa. Amp: Adversarial motion priors
for stylized physics-based character control. ACM Transactions on Graphics (ToG), 40(4):
1–20, 2021.
[45] B. Jiang, X. Chen, W. Liu, J. Yu, G. Yu, and T. Chen. Motiongpt: Human motion as a foreign
language. Advances in Neural Information Processing Systems, 36, 2024.
[46] S. Kuindersma, R. Deits, M. Fallon, A. Valenzuela, H. Dai, F. Permenter, T. Koolen, P. Marion,
and R. Tedrake. Optimization-based locomotion planning, estimation, and control design for
the atlas humanoid robot. Autonomous robots, 40:429–455, 2016.
13
[47] Y. Liang, W. Li, Y. Wang, R. Xiong, Y. Mao, and J. Zhang. Dynamic movement primitive
based motion retargeting for dual-arm sign language motions. In 2021 IEEE International
Conference on Robotics and Automation (ICRA), pages 8195–8201. IEEE, 2021.
[48] S. Caelles, J. Pont-Tuset, F. Perazzi, A. Montes, K.-K. Maninis, and L. Van Gool. The
2019 davis challenge on vos: Unsupervised multi-object segmentation. arXiv preprint
arXiv:1905.00737, 2019.
[49] Y. Huang, J. Yuan, C. Kim, P. Pradhan, B. Chen, L. Fuxin, and T. Hermans. Out of sight,
still in mind: Reasoning and planning about unobserved objects with video tracking enabled
memory models. arXiv preprint arXiv:2309.15278, 2023.
[50] Y. Zhu, Z. Jiang, P. Stone, and Y. Zhu. Learning generalizable manipulation policies with
object-centric 3d representations. In 7th Annual Conference on Robot Learning, 2023.
[51] A. Stone, T. Xiao, Y. Lu, K. Gopalakrishnan, K.-H. Lee, Q. Vuong, P. Wohlhart, S. Kirmani,
B. Zitkovich, F. Xia, et al. Open-world object manipulation using pre-trained vision-language
models. arXiv preprint arXiv:2303.00905, 2023.
[52] H. K. Cheng, S. W. Oh, B. Price, J.-Y. Lee, and A. Schwing. Putting the object back into video
object segmentation. In arXiv, 2023.
[53] V. Ye, G. Pavlakos, J. Malik, and A. Kanazawa. Decoupling human and camera motion from
videos in the wild. In CVPR, 2023.
[54] M. Loper, N. Mahmood, J. Romero, G. Pons-Moll, and M. J. Black. Smpl: A skinned multi-
person linear model. In Seminal Graphics Papers: Pushing the Boundaries, Volume 2, pages
851–866. 2023.
[55] J. Rajasegaran, G. Pavlakos, A. Kanazawa, and J. Malik. Tracking people by predicting 3d
appearance, location and pose. In Proceedings of the IEEE/CVF Conference on Computer
Vision and Pattern Recognition, pages 2740–2749, 2022.
[56] J. Romero, D. Tzionas, and M. J. Black. Embodied hands. ACM Transactions on Graphics, 36
(6):1–17, 2017.
[57] G. Pavlakos, D. Shan, I. Radosavovic, A. Kanazawa, D. Fouhey, and J. Malik. Reconstructing
hands in 3D with transformers. In CVPR, 2024.
[58] N. Karaev, I. Rocco, B. Graham, N. Neverova, A. Vedaldi, and C. Rupprecht. Cotracker: It is
better to track together. arXiv preprint arXiv:2307.07635, 2023.
[59] R. Killick, P. Fearnhead, and I. A. Eckley. Optimal detection of changepoints with a linear
computational cost. Journal of the American Statistical Association, 107(500):1590–1598,
2012.
[60] Q.-Y. Zhou, J. Park, and V. Koltun. Open3d: A modern library for 3d data processing. arXiv
preprint arXiv:1801.09847, 2018.
[61] Y. Zhu, J. Wong, A. Mandlekar, R. Mart´ın-Mart´ın, A. Joshi, S. Nasiriany, and Y. Zhu. ro-
bosuite: A modular simulation framework and benchmark for robot learning. arXiv preprint
arXiv:2009.12293, 2020.
[62] T. Z. Zhao, V. Kumar, S. Levine, and C. Finn. Learning fine-grained bimanual manipulation
with low-cost hardware. arXiv preprint arXiv:2304.13705, 2023.
[63] S. Goel, G. Pavlakos, J. Rajasegaran, A. Kanazawa, and J. Malik. Humans in 4D: Reconstruct-
ing and tracking humans with transformers. In ICCV, 2023.
14
[64] Y. Xu, J. Zhang, Q. Zhang, and D. Tao. ViTPose++: Vision transformer for generic body pose
estimation. IEEE Transactions on Pattern Analysis and Machine Intelligence, 2023.
[65] S. Caron, Y. De Mont-Marin, R. Budhiraja, and S. H. Bang. Pink: Python inverse kinematics
based on Pinocchio, 2024. URL https://github.com/stephane-caron/pink.
[66] Y. Qin, W. Yang, B. Huang, K. Van Wyk, H. Su, X. Wang, Y.-W. Chao, and D. Fox. Anyteleop:
A general vision-based dexterous robot arm-hand teleoperation system. In Robotics: Science
and Systems, 2023.
[67] X. Cheng, J. Li, S. Yang, G. Yang, and X. Wang. Open-television: Teleoperation with immer-
sive active visual feedback. arXiv preprint arXiv:2407.01512, 2024.
[68] T. Darcet, M. Oquab, J. Mairal, and P. Bojanowski. Vision transformers need registers, 2023.
[69] M. Oquab, T. Darcet, T. Moutakanni, H. V. Vo, M. Szafraniec, V. Khalidov, P. Fernandez,
D. Haziza, F. Massa, A. El-Nouby, R. Howes, P.-Y. Huang, H. Xu, V. Sharma, S.-W. Li,
W. Galuba, M. Rabbat, M. Assran, N. Ballas, G. Synnaeve, I. Misra, H. Jegou, J. Mairal,
P. Labatut, A. Joulin, and P. Bojanowski. Dinov2: Learning robust visual features without
supervision, 2023.
15
A Implementation Details
A.1 Human Reconstruction From Videos
Method. For the 3D human reconstruction, we start by tracking the person in the video and getting
an initial estimate of their 3D body pose using 4D Humans [63]. This body reconstruction cannot
capture the hand pose details (i.e., the hands are flat). Therefore, for each detection of the person in
the video, we detect the two hands using ViTPose [64], and for each hand, we apply HaMeR [57]
to get an estimate of the 3D hand pose. However, the hands reconstructed by HaMeR can be incon-
sistent with the arms from the body reconstruction (e.g., different wrist orientation and location).
To address this, we apply an optimization refinement to make the body and the hands consistent in
each frame, and encourage that the holistic body and hands motion is smooth over time. This op-
timization is similar to SLAHMR [53], with the difference that besides the body pose and location
of the SMPL+H model [56], we also optimize the hand poses. We initialize the procedure using the
3D body pose estimate from 4D Humans and the 3D hand poses from HaMeR. Moreover, we use
the 2D projection of the 3D hands predicted by HaMeR to constrain the projection of the 3D hand
keypoints of the holistic model using a reprojection loss. Finally, we can jointly optimize all the
parameters (body location, body pose, hand poses) over the duration of the video, as described in
SLAHMR [53].
Inference Requirements. The model of human reconstruction we use is large and needs to be run
on a computer with sufficiently good computation speed. Here we provide details about the runtime
performance of the human reconstruction model. We use a desktop that comes with a GPU RTX3090
that has the size of the memory 24 GB. For a 10 seconds video with fps 30, it processes 10 minutes.
A.2 Prompts of Using GPT4V
In order to use GPT4V in OKAMI, we need GPT4V’s output to be in a typed format so that the
rest of the programs can parse the result. Moreover, in order for the prompts to be general across a
diverse set of tasks, our prompt does not leak any task information to the model. Here we describe
the three different prompts in OKAMI for using GPT4V.
Identify Task-relevant Objects. OKAMI uses the following prompt to invoke GPT4V so that it
can identify the task-relevant objects from a provided human video:
Prompt: You need to analyze what the human is doing in the images, then tell me: 1. All the
objects in front scene (mostly on the table). You should ignore the background objects. 2. The
objects of interest. They should be a subset of your answer to the first question. They are likely
the objects manipulated by human or near human. Note that there are irrelevant objects in the
scene, such as objects that does not move at all. You should ignore the irelevant objects.
Your output format is:
The human is xxx.
All objects are xxx.
The objects of interest are:
‘‘‘
json
{
"objects": ["OBJECT1", "OBJECT2", ...],
}
‘‘‘
Ensure the response can be parsed by Python ‘json.loads’, e.g.: no trailing commas, no single
quotes, etc. You should output the names of objects of interest in a list [“OBJECT1”, “OB-
JECT2”, ...] that can be easily parsed by Python. The name is a string, e.g., “apple”, “pen”,
“keyboard”, etc.
16
Identify Target Objects. OKAMI uses the following prompt to identify the target object of each
step in the reference plan:
Prompt: The following images shows a manipulation motion, where the human is manipulating
an object.
Your task is to determine which object is being manipulated in the images below. You need to
choose from the following objects: {a list of task-relevant objects}.
Tips: the manipulated object is the object that the human is interacting with, such as picking up,
moving, or pressing, and it is in contact with the human’s {the major moving arm in this step}
hand.
Your output format is:
‘‘‘json
{
"manipulate_object_name": "MANIPULATE_OBJECT_NAME",
}
‘‘‘
Ensure the response can be parsed by Python ‘json.loads’, e.g.: no trailing commas, no single
quotes, etc.
Identify Reference Objects. Here is the prompt that asks GPT4V to identify the reference object
of each step in the reference plan:
Prompt: The following images shows a manipulation motion, where the human is manipulating
the object {manipulate object name}.
Please identify the reference object in the image below, which could be an object on which
to place {manipulate object name}, or an object that {manipulate object name} is interacting
with. Note that there may not necessarily have an reference object, as sometimes human may
just playing with the object itself, like throwing it, or spinning it around. You need to first
identify whether there is a reference object. If so, you need to output the reference object’s
name chosen from the following objects: {a list of task-relevant objects}.
Your output format is:
‘‘‘json
{
"reference_object_name": "REFERENCE_OBJECT_NAME" or "None",
}
‘‘‘
Ensure the response can be parsed by Python ‘json.loads’, e.g.: no trailing commas, no single
quotes, etc.
A.3 Details on Factorized Process for Retargeting
Body Motion Retarget. To retarget body motions from the SMPL-H representation to the hu-
manoid, we extract the shoulder, elbow, and wrist poses from the SMPL-H models. We then use
inverse kinematics to solve the body joints on the humanoid, ensuring they produce similar shoulder
and elbow orientations and similar wrist poses. The inverse kinematics is implemented using an
open-sourced library Pink [65]. The IK weights we use for shoulder orientation, elbow orientation,
wrist orientation, and wrist position are 0.04, 0.04, 0.1, and 1.0, respectively.
Hand Pose Mapping. As we describe in the method section, we first retarget the hands from
SMPL-H models to the humanoid’s dexterous hands using a hybrid implementation of inverse kine-
matics and angle mapping. Here are the details of how this mapping is performed. Once we obtain
17
the SMPL-H models from a video demonstration, we can obtain the locations of 3D joints from the
hand mesh models from SMPL-H. Subsequently, we can compute the rotating angles of each joint
that correspond to certain hand poses. Then we apply the computed joint angles to the hand meshes
of a canonical SMPL-H model, which is pre-defined to have the same size as the humanoid robot
hardware. From this canonical SMP-H model, we can get the 3D keypoints of hand joints and use an
existing package, dex-retarget, an off-the-shelf optimization package to directly compute the hand
joint angles of the robot [66].
A.4 Trajectory Warping
Here, we mathematically describe the process of trajectory warping. We denote the trajectory for
robot as τ robot retargeted from τ SMPL
ti:ti+1 in the generated plan. Denote the starting point and end point
of τ robot as pstart, pend, respectively. Note that all points along the trajectory are represented in SE(3)
space.
Each point pt on the original retargetd trajectory can be described by the following function:
pt = pstart + (τ robot(t) − pstart) (1)
where t ∈ {ti, . . . , ti+1}, τ robot(ti) = pstart, τ robot(ti+1) = pend.
When warping the trajectory, we either only needs to adapt the trajectory to the new target object
location, or adapt the trajectory to the new locations of both the target and the reference objects,
as described in Section 3.3. Without loss of generality, we denote the SE(3) transformation for
the starting point is Tstart, and the SE(3) transformation for the end point is Tend. Now the warped
trajectory can be described by the following function:
pt = Tstart · pstart + (ˆτ robot(t) − Tstart · pstart) (2)
where ˆτ robot(t) = τ robot(t)−pstart
pend−pstart (Tend ·pend −Tstart ·pstart)+Tstart ·pstart, ∀t ∈ {ti, . . . , ti+1}. In this way,
we have ˆτ robot(ti) = Tstart · pstart, ˆτ robot(ti+1) = Tend · pend. Note that this trajectory warping assumes
the end point of a trajectory is not the same as the starting point, which is a common assumption for
most of the manipulation behaviors.
B Additional Experimental Details
B.1 Success Conditions
We describe the success conditions we use to evaluate if a task rollout is successful or not.
• Sprinkle-salt: The salt bottle reaches a position where the salt is poured out into the
bowl.
• Plush-toy-in-basket: The plush toy is put inside the container, with more than 50%
of the toy inside the container.
• Close-the-laptop: The display is lowered towards the base until the two parts meet
at the hinge (aka the laptop is closed).
• Close-the-drawer: The drawer is pushed back to the containing region, either it’s a
drawer or a layer of a cabinet.
• Place-snacks-on-plate: The snack is placed on top of the plate, with more than
50%
• Bagging: The chip bag is put into the shopping bag which is initially closed.
B.2 Implementation of Baseline
We implement the baseline ORION [4] with minimal modifications to apply it to our humanoid
setting. First, we estimate the palm trajectory from SMPL-H trajectories by using the center point of
18
Figure 6: The initial and end frames of videos performed by different human demonstrators. The first row is
Place-snacks-on-plate task, and the second row is Close-the-laptop task.
the reconstructed fingers as the palm position at each time step. Next, we warp the palm trajectory
based on the test-time objects’ locations. Finally, we use inverse kinematics to solve for the robot’s
body joints, with the warped trajectory serving as the target palm position.
B.3 Details on Different Demonstrators
Figure 6 shows the videos of three different human demonstrators performing
Place-snacks-on-plate and Close-the-laptop tasks. We calculate the success
rates of imitating different videos, and the results are shown in Figure 4(b).
B.4 Simulation Evaluation
For easy reproducibility, we replicate two tasks, Sprinkle-salt and Close-the-drawer,
in simulation (Figure 7). We implement these tasks using robosuite [61], which recently provided
cross-embodiment support, including humanoid manipulation. We use “GR1FixedLowerBody” as
the robot embodiment in these two tasks.
Note that for the policy of each task, we use the same human video as the ones used in real robot
experiments. We compare three methods in simulation: OKAMI (w/vision), OKAMI (w/o vision),
and ORION. OKAMI (w/vision) the same method we use in our real robot experiments. OKAMI
(w/o vision) is the simplified version of OKAMI where we assume the model directly gets the
ground-truth poses of objects. The evaluation results are shown in Table 1, where each reported
number is the success rate averaged over 50 rollouts.
We notice that the simulation results are generally better than the real robot experiments. The per-
formance difference is comes from easy physical interaction between dexterous hands and objects
compared to the real robot hardware. Also, OKAMI without vision can achieve much higher suc-
cess rate than OKAMI with vision because the noise and uncertainty of perception is abstracted
19
Close-the-drawer Sprinkle-saltFigure 7: The screenshots of the starting and ending frames of the two simulation tasks, Close-the-drawer
and Sprinkle-salt.
away. Specifically, a large portion of uncertainties come from the partial observation of object point
clouds, and the estimation of the object location is off the ground-truth locations of objects, while the
success of OKAMI highly depends on the quality of trajectory warping, which is dependent on the
correct estimation of object locations. This simulation result also indicates that the performance of
OKAMI is expected to improve if more powerful vision models with higher accuracy are available.
Method Sprinkle-salt Close-the-drawer
OKAMI (w/ vision) 82%
OKAMI (w/o vision) 100%
ORION 0%
Table 1: The average success rates (%
Close-the-drawer
B.5 Visuomotor Policy Details
We choose ACT [62] in our experiments for behavioral cloning, an algorithm which has been
shown effective in learning humanoid manipulation policies [67]. Notably, we choose pretrained
DinoV2 [68, 69] as the visual backbone of a policy. The policy takes a single RGB image and 26-
dimension joint positions as input and outputs the action of the 26-dimension absolute joint position
for the robot to reach. In Table 2, we show the hyperparameters used for behavioral cloning.
KL weight 10
chunk size 60
hidden dimension 512
batch size 45
feedforward dimension 3200
epochs 25000
learning rate 5e-5
temporal weighting 0.01
Table 2: The hyperparameters used in ACT.
20

